Early Detection of Bark Beetle Attack Using Remote Sensing and Machine Learning: A Review

This paper provides a comprehensive review of past and current advances in the early detection of bark beetle-induced tree mortality from three primary perspectives: bark beetle & host interactions, RS, and ML/DL. In contrast to prior efforts, this review encompasses all RS systems and emphasizes ML/DL methods to investigate their strengths and weaknesses. We parse existing literature based on multi- or hyper-spectral analyses and distill their knowledge based on: bark beetle species & attack phases with a primary emphasis on early stages of attacks, host trees, study regions, RS platforms & sensors, spectral/spatial/temporal resolutions, spectral signatures, spectral vegetation indices (SVIs), ML approaches, learning schemes, task categories, models, algorithms, classes/clusters, features, and DL networks & architectures. Although DL-based methods and the random forest (RF) algorithm showed promising results, highlighting their potential to detect subtle changes across visible, thermal, and short-wave infrared (SWIR) spectral regions, they still have limited effectiveness and high uncertainties. To inspire novel solutions to these shortcomings, we delve into the principal challenges & opportunities from different perspectives, enabling a deeper understanding of the current state of research and guiding future research directions.

==> Table_Software.tex <==
\begin{table*}[!tp]
\rowcolors{2}{}{gray!10}
\caption{Pre-processing software tools assisting in the detection of bark beetle attacks.} % title of Table
\centering 
 \resizebox{\textwidth}{!}{
\begin{tabular}{c c c} % centered columns (4 columns)
\hline
Software & Description & URL  \protect\\ 
\hline\hline
%   &   &   &   &
ImageStation &  High Volume Photogrammetry and Production Mapping  & \href{https://www.hexagongeospatial.com/products/power-portfolio/imagestation}{Link}     \protect\\ 

ERDAS Imagine    & \thead{Remote sensing, photogrammetry, LiDAR analysis, \\ basic vector analysis, and radar processing }     &   \href{https://www.hexagongeospatial.com/products/power-portfolio/erdas-imagine}{Link}       \protect  \\

%---------------------------------------------------------------------------------------
ENVI     &  Industry standard for image processing and analysis software   &  \href{https://www.l3harrisgeospatial.com/Software-Technology/ENVI?gclid=Cj0KCQiAjJOQBhCkARIsAEKMtO2LQToUWz-iCDcmPiB1kjC31wnz_f5hLoiVbKhsRe_AOj9QeNXBeiAaAq15EALw_wcB}{Link}         \protect  \\

METRO  &  Elimination of Terrain and Relief Displacement in Orthophotography  &  \href{https://www.sanborn.com/applications-for-our-services/}{Link}         \protect  \\

% ACORN      &   \href{}{Link}    &        \protect  \\

ATCOR     &  Atmospheric/topographic correction   &   \href{https://www.rese-apps.com/software/atcor/index.html}{Link}         \protect  \\

% ORTHO    &    \href{}{Link}   &        \protect  \\

% Exelis Visual Information Solutions      &    \href{}{Link}   &        \protect  \\

GAMMA     &  \thead{Processing chain (Synthetic Aperture Radar (SAR) raw data to end products, \\ e.g., DEMs, displacement maps \& land use maps)}    &  \href{https://www.gamma-rs.ch/software}{Link}        \protect  \\

GENIE      &  \thead{Automatic feature extraction in multispectral, hyperspectral, \\ panchromatic, and multi-instrument fused imagery}   &   \href{http://observera.com/solutions/genie-pro/}{Link}       \protect  \\

RapidMiner    &  Data science platform     &   \href{https://rapidminer.com/}{Link}       \protect  \\

FUSION   &  Analyze LiDAR data     &  \href{http://forsys.cfr.washington.edu/FUSION/fusion_overview.html}{Link}         \protect  \\

BCAL    & Processing, analyzing and visualizing LiDAR data      &   \href{https://www.boisestate.edu/bcal/resources/bcal-lidar-tools/}{Link}       \protect  \\

Quantum GIS (QGIS)    &  Geographic Information System      &  \href{https://www.qgis.org/en/site/}{Link}       \protect  \\
%---------------------------------------------------------------------------------------
ArcGIS  &  Identify spatial patterns, trends, and non-obvious relationships   &  \href{https://www.esri.com/en-us/arcgis/about-arcgis/overview}{Link}       \protect  \\

Web-GIS      &   \thead{Pattern, or architectural approach for implementing \\ a modern GIS (web services—standard services)}     &  \href{https://www.esri.com/about/newsroom/insider/web-gis-simply/}{Link}   \protect  \\

StereoAnalyst    & Stereo Photogrammetry for ArcGIS    &   \href{https://www.geosystems.de/en/products/stereo-analystr}{Link}         \protect  \\
%---------------------------------------------------------------------------------------
JMP Statistical Software     &  Statistical Software     &  \href{https://www.jmp.com/en_ca/home.html}{Link}       \protect  \\

ViewSpec Pro      & Post-processing spectra files    &   \href{https://www.malvernpanalytical.com/en/support/product-support/software/ViewSpecProSoftwareInstall.html}{Link}       \protect  \\
      
GDAL     & Translator library for raster and vector geospatial data formats   &   \href{https://gdal.org/}{Link}         \protect  \\
      
LAStools      &  Software for rapid LiDAR processing   &  \href{http://lastools.org/}{Link}        \protect  \\
      
Agisoft      & Photogrammetric processing of digital images and generates 3D spatial data     &  \href{https://www.agisoft.com/}{Link}       \protect  \\
      
eCognition      &  Interpretation of geospatial data products by designing feature extraction and change detection     &    \href{https://www.geospatial.trimble.com/products-and-solutions/ecognition}{Link}     \protect  \\
      
Systat      &  Statistical Analysis and Graphics Software    &   \href{https://systatsoftware.com/systat/}{Link}      \protect  \\
      
MODTRAN4    &  Atmospheric correction, in remotely sensed multi- and hyperspectral imaging (MSI and HSI)    &  \href{http://modtran.spectral.com/}{Link}         \protect  \\
      
SEN2COR       &   Processor for Sentinel-2 Level 2A product generation and formatting(atmospheric correction, etc.)  &  \href{https://step.esa.int/main/snap-supported-plugins/sen2cor/}{Link}        \protect  \\
      
STATISTICA      & Statistical, predictive, data mining, machine learning, forecasting, optimization, and text analytic models     &  \href{https://docs.tibco.com/products/tibco-statistica-14-0-0}{Link}       \protect  \\
      
FLAASH     &  Atmosphere Correction    &  \href{https://www.spectral.com/our-software/flaash/}{Link}        \protect  \\
      
Headwall's SpectralView      & Hyperspectral and Operational Software    &  \href{https://www.headwallphotonics.com/products/software}{Link}        \protect  \\

TANABBO      &  \thead{Process 3D points clouds and extract high resolution DEM, DSM,\\ classify point clouds, measure and model individual trees }    &   \href{http://gis.tuzvo.sk/dendrocloud/}{Link}     \protect  \\
      
BioSIM        &  Temperature-driven simulation models in pest management  &  \href{https://cfs.nrcan.gc.ca/projects/133}{Link}       \protect  \\
      
ORFEO Toolbox     &  Process high resolution optical, multispectral and radar images at the terabyte scale   &  \href{https://www.orfeo-toolbox.org/}{Link}        \protect  \\
      
Pix4Dmapper      &  Photogrammetry software for professional drone mapping     &  \href{https://www.pix4d.com/product/pix4dmapper-photogrammetry-software}{Link}      \protect  \\
      
TerraSolid    & Industry standard software for point cloud and image processing     &   \href{https://terrasolid.com/}{Link}        \protect  \\
      
SAGA GIS      &  GIS software (spatial algorithms implementation, geoscientific methods, visualisation options)    &  \href{https://saga-gis.sourceforge.io/en/index.html}{Link}       \protect  \\
      
% FGI      &  \href{}{Link}    &         \protect  \\
      
% RadBA      &  \href{}{Link}     &        \protect  \\
      
PCI geomatica     &  \thead{Geo-image software (remote sensing, digital photogrammetry, \\ image analysis, map production, mosaicking, etc.)}    &    \href{https://catalyst.earth/about/}{Link}    \protect  \\
      
Py6S      &  Simulation of the Satellite Signal in the Solar Spectrum (6S) atmospheric Radiative Transfer Model     &    \href{https://py6s.readthedocs.io/en/latest/}{Link}    \protect  \\
      
SNAP     & Scientific exploitation for the ERS-ENVISAT missions (e.g., Sentinels 1/2/3)    &   \href{http://step.esa.int/main/}{Link}       \protect  \\
      
OpenDroneMap     &  Collecting, processing, analyzing and displaying aerial data      &  \href{https://www.opendronemap.org/}{Link}      \protect  \\
      
ImageMagic      &  Create, edit, compose, or convert digital images   &   \href{https://imagemagick.org/}{Link}       \protect  \\
      
Spectronon    & \thead{Control Resonon's benchtop and outdoor hyperspectral imaging \\ systems (data processing, analysis, \& visualization tools) }     &   \href{https://resonon.com/software}{Link}      \protect  \\
      
LiDAR360     &  Point Cloud Post-Processing Software   &   \href{https://greenvalleyintl.com/LiDAR360/}{Link}        \protect  \\
      
GRASS GIS      &  Geographic Resources Analysis     &  \href{https://grass.osgeo.org/}{Link}      \protect  \\
      
% EU-DEM 25      &    \href{}{Link}   &        \protect  \\
    
GIMP     &  Image Manipulation Program       &  \href{https://www.gimp.org/}{Link}      \protect  \\
      
Global Mapper    &  GIS software with spatial data processing tools and unparalleled variety of data formats     &    \href{https://www.bluemarblegeo.com/global-mapper/}{Link}      \protect  \\
      
DJI Terra     & Capture, analyze and visualize your environment     &  \href{https://www.dji.com/ca/dji-terra}{Link}        \protect  \\
      
DJI GS Pro \& Terra   &  Automated flight missions, manage flight data on the cloud, and collaborate across projects      &  \href{https://www.dji.com/ca/ground-station-pro}{Link}        \protect  \\      
  
%---------------------------------------------------------------------------------------
\hline 
\end{tabular}
  \label{tab_Software}  
  }
\end{table*}

==> Table_SpectralBands.tex <==
\begin{table*}[!tbp]
\rowcolors{2}{}{gray!10}
\caption{Spectral bands and their characteristics.} % title of Table
\centering 
 \resizebox{\textwidth}{!}{
\begin{tabular}{c  c | c | c | c}
\hline\hline

\multicolumn{2}{c|}{Spectral band} & Wavelength range ($\mu m$) & Radiation source & Surface property \\ \hline

\cellcolor{gray!10} & Violet & $0.4 - 0.45$ & \cellcolor{gray!10}  & \cellcolor{gray!10}  \\ 

\cellcolor{gray!10} & \cellcolor{gray!10} Blue & \cellcolor{gray!10} $0.45-0.5$ & \cellcolor{gray!10} & \cellcolor{gray!10}  \\ 

\cellcolor{gray!10} & \cellcolor{gray!10} Green & \cellcolor{gray!10} $0.5-0.6$ & \cellcolor{gray!10}  & \cellcolor{gray!10}  \\ 

\multirow{-4}{*}{\cellcolor{gray!10}Visible} & \cellcolor{gray!10} Red & \cellcolor{gray!10} $0.6-0.7$ & \multirow{-4}{*}{\cellcolor{gray!10} Solar} & \multirow{-4}{*}{\cellcolor{gray!10} Reflectance} \\ 

\multicolumn{2}{c|}{\global\let\CT@@do@color\relax Red-edge} & $0.7-0.8$ & Solar & Reflectance  \\ 

\multicolumn{2}{c|}{\global\let\CT@@do@color\oriCT@@do@color \cellcolor{gray!10} Near Infrared (NIR)} & \cellcolor{gray!10} $0.7-1$ & \cellcolor{gray!10} Solar & \cellcolor{gray!10} Reflectance \\ 

\multicolumn{2}{c|}{\global\let\CT@@do@color\relax Short-wave Infrared (SWIR)} & $1-3$ & Solar & Reflectance \\ 

\global\let\CT@@do@color\oriCT@@do@color \cellcolor{gray!10}  & \cellcolor{gray!10} Mid-wave Infrared (MWIR) & \cellcolor{gray!10} $3-5$ & \cellcolor{gray!10} Solar, Thermal & \cellcolor{gray!10} Reflectance, Temperature \\  

\multirow{-2}{*}{\cellcolor{gray!10} Thermal Infrared (TIR)} & Long-wave Infrared (LWIR) & $8-14$ & Thermal & Temperature \\ \hline

\end{tabular}
  \label{tab_SpectralBands}  
} 
\end{table*} 

% \global\let\CT@@do@color\oriCT@@do@color
